NimbRo-OP2X: Affordable Adult-sized 3D-printed Open-Source Humanoid Robot for Research

For several years, high development and production costs of humanoid robots restricted researchers interested in working in the field. To overcome this problem, several research groups have opted to work with simulated or smaller robots, whose acquisition costs are significantly lower. However, due to scale differences and imperfect simulation replicability, results may not be directly reproducible on real, adult-sized robots. In this paper, we present the NimbRo-OP2X, a capable and affordable adult-sized humanoid platform aiming to significantly lower the entry barrier for humanoid robot research. With a height of 135 cm and weight of only 19 kg, the robot can interact in an unmodified, human environment without special safety equipment. Modularity in hardware and software allow this platform enough flexibility to operate in different scenarios and applications with minimal effort. The robot is equipped with an on-board computer with GPU, which enables the implementation of state-of-the-art approaches for object detection and human perception demanded by areas such as manipulation and human-robot interaction. Finally, the capabilities of the NimbRo-OP2X, especially in terms of locomotion stability and visual perception, are evaluated. This includes the performance at RoboCup 2018, where NimbRo-OP2X won all possible awards in the AdultSize class.

==> commentedbib.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


==> letter/addon/commands-for-letter-to-reviewers.tex <==
%
%
\RequirePackage{ifdraft}
%
\RequirePackage{xcolor}
%
\RequirePackage{cleveref}
%
\geometry{
 a4paper,
 total={210mm,297mm},
 left=15mm,
 right=15mm,
 top=15mm,
 bottom=25mm,
 marginparwidth=15mm
}
%
\renewcommand\Affilfont{\itshape\small}

%
\newcounter{commentcnt}[section]
%
\renewcommand{\thecommentcnt}{\Roman{commentcnt}}
%
\Crefname{commentcnt}{Comment}{Comment}

\newenvironment{ReviewerComment}[2][]{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} %
%
\ifx\empty#1\relax\else#1\fi%
(Reviewer #2): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{ReviewerCommentReprise}{\noindent\vspace{-1.25cm}%
\begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}}
%
\newenvironment{ReviewerReply}{\noindent \textbf{Feedback: } \begin{quotation}\begin{em}}{\end{em}\end{quotation}}
%
\newenvironment{GuestEditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Guest Editor): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{AreaEditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Area Editor): }\nopagebreak \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{EditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} : } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{MetaReviewComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Meta-review): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{Answer}{\noindent \textbf{Answer: }}{\\[1cm]}
%
\newenvironment{AnswerInBetween}{\noindent \textbf{Answer: }}{\vspace{1cm}}
%
%


\newcommand{\NoteInEvidence}[1]{\ifoptiondraft{\hl{#1}}{}}

%
%
%
%
%
\newcommand{\TaskEstimationBox}[2]{%
\ifoptiondraft{\newline \parbox{1.0\linewidth}{\hfill \hfill {\colorbox{#2}{\color{White} \textbf{#1}}}}}%
{}%
}
%
\def\WorkInProgressRevTask {\TaskEstimationBox{Work in progress}{Cyan}}
\def\AlmostDoneRevTask {\TaskEstimationBox{Almost there}{NavyBlue}}
\def\RevTaskDone {\TaskEstimationBox{Done}{Blue}}
%
\def\NotEstimatedRevTask {\TaskEstimationBox{Effort not estimated}{Gray}}
\def\EasyRevTask {\TaskEstimationBox{Feasible}{ForestGreen}}
\def\MediumRevTask {\TaskEstimationBox{Medium effort}{Orange}}
\def\TimeConsumingRevTask {\TaskEstimationBox{Time-consuming}{Bittersweet}}
\def\HardRevTask {\TaskEstimationBox{Hard one}{Sepia}}
\def\DeathRevTask {\TaskEstimationBox{Death}{Black}}
%
\newcommand{\Assignment}[1]{
%
\ifoptiondraft{%
\newline \parbox{1.0\linewidth}{\hfill \hfill \textbf{Assignment:} #1}%
}{}%
}

%
%
%
\newcommand{\SkipSpaceForReviewerComments}{\vspace{6em}}

%
%
%
%
\RequirePackage{xcolor}
\newenvironment{NoteForAuthors}%
  {\ifoptiondraft{%
      \noindent%
      \colorbox{gray}%
      {\color{white} Note: }%
      \color{orange}%
      \begin{em}%
    }{}%
  }%
  {\ifoptiondraft{%
      \normalcolor%
      \end{em}%
    }{}%
  }

%
%
%
%
\RequirePackage{xcolor}
%
\RequirePackage{marginnote}
%
\setlength{\marginparwidth}{1cm}
%
\renewcommand*{\marginfont}{\footnotesize}

\newenvironment{HlRev}[1][]{%
	%
	\begin{NoHyper}
		%
		\color{OliveGreen}%
		%
		\ifx\newenvironment#1\newenvironment\else\marginnote{Comment #1}\fi%
		%
	}{%
		%
		\normalcolor%
		%
	\end{NoHyper}%
}
%
%
%


==> letter/addon/pkgloading-for-letter-to-reviewers.tex <==
%
\usepackage[usenames,dvipsnames]{xcolor}
%
\usepackage{url}
%
\usepackage{paralist}
%
\usepackage[obeyDraft,textsize=tiny,backgroundcolor=blue!10]{todonotes}
%
%
%
\usepackage{authblk}
%
%
%
\usepackage{enumitem}
%
\usepackage[british]{babel}
%
\usepackage{marvosym}
%
\usepackage{comment}
%
\usepackage{geometry}
%
\usepackage[implicit=false]{hyperref}
%
\usepackage{enumitem}
%
\usepackage{amsfonts}
%
\usepackage{marginnote}
%
\usepackage[nonumberlist,acronym,sanitize=none]{glossaries}
\glsdisablehyper
%
\usepackage{amsmath}
%
\usepackage{mathrsfs}
%
\usepackage{amssymb}
%
\usepackage{ifdraft}
%
\usepackage{soul}
%
\usepackage{siunitx}
%
\usepackage{textcomp}
%
\usepackage[capitalise,nameinlink]{cleveref}
%
\usepackage{xr}

==> letter/intro.tex <==
Dear Dr.\ Ming Xie
\\[2em]
We express our gratitude for the time and effort dedicated to the reviewing and processing of our submitted manuscript. 
We worked diligently to address all the concerns raised by the reviewers. As only Reviewer 3 made suggestions 
to improve the content of the article, we have omitted the comment of Reviewer 1. Below we provide our detailed response to these comments.

We hope that the applied revisions are to the satisfaction of the editors.\\

For any questions, please contact us at \texttt{ficht@ais.uni-bonn.de.}\\
\\[1em]
Kind regards,
\begin{flushright}
\begin{tabular}{lll}
    Ficht Grzegorz, Hafez Farazi, Diego Rodriguez, Dmytro Pavlichenko, Philipp Allgeuer, Andr\'e Brandenburger, and Sven Behnke.
\end{tabular}
\end{flushright}


==> letter/manuscriptinfo.tex <==
\section*{Manuscript information}

\begin{description}
\item[Number:] \PaperId
\item[Title:] ``\PaperTitle''
%
\item[Submitted to:] \Journal
\item[Special issue:] \SpecialIssueId
\end{description}

==> letter/revision-notes/report.tex <==
%
%
%
%
\section*{Report}

%
%
\begin{EditorComment}
As only Reviewer 3 provided his remarks, the letter will 
\end{EditorComment}
%
\begin{Answer} 
Bla
\end{Answer}
%
%


==> letter/revision-notes/reviewer1.tex <==
%
%
%
%
\setcounter{commentcnt}{0}
\section*{Reviewer 1}
%
%
\begin{ReviewerComment}{1}
Bla
\end{ReviewerComment}
%
\begin{Answer} 
Bla
\end{Answer}
%
%
%
%
\begin{ReviewerComment}{1}
Bla
\end{ReviewerComment}
%
\begin{Answer}
Bla
\end{Answer}


==> letter/revision-notes/reviewer2.tex <==
%
%
%
%
\setcounter{commentcnt}{0}
\section*{Reviewer 3}
%
%
%
%

%
%
\begin{ReviewerComment}{3}
This paper could benefit from incorporation of more technical information, such as the equations governing the locomotion algorithms, which would probably even reduce the length of the text. Prolix descriptions are used in some cases, which could easily be replaced by mathematical formulae (section 4 in particular).\end{ReviewerComment}
%
\begin{Answer}
Equations have been added specifically to the gait section to describe the abstract pose space and its conversion to joint space, as that does add clarity to how the trajectories are generated. It was also not our intention to re-state what was already written in the publication by Allgeuer and Behnke: ``Omnidirectional Bipedal Walking with Direct Fused Angle Feedback Mechanisms'' (which is referenced in the gait section), but provide a more intuitive  description of how the gait works. More specific explanations to the mechanisms mentioned in further comments have been addressed.
\end{Answer}
%
%

%
%
\begin{ReviewerComment}{3}
It would also be useful to delineate the mechanics of the 'CoM shifting' process, which the reader is currently led to believe, may even be performed in a heuristic manner. Is a simplified model used to regulate the CoM position in real time?
\end{ReviewerComment}
%
\begin{Answer}
The whole set of corrective actions are indeed heuristics, which the text now clearly states:

``The walking algorithm of the NimbRo-OP2X is based on producing joint trajectories 
that result in a semi-stable open-loop walking gait, and then 
to stabilize this gait through integration of multiple heuristics, called \textit{corrective actions}. 
This results in a modification of the gait trajectories in order to specifically affect the balance in a targeted way. ''

The CoM shifting process has also been described in more detail:

``The inverse kinematic position of the feet relative to the torso are adjusted in the horizontal plane relative to the torso. As the CoM of the robot is assumed to be situated at a constant offset relative to the torso frame, this results in shifting the position of the assumed CoM over the robots support polygon.''
\end{Answer}
%
%

%
%
\begin{ReviewerComment}{3}
A similar comment can be made about the methodology described on page 15, which entails superimposition of several PD-type controllers relying upon manually-tuned gains (or gains that have been selected via simulation). It would also be interesting to elaborate on the operation of the 'speed-up and slow-down gains', as this could be of practical significance to anybody either purchasing a NimbRo-OP2X unit, or developing an analogous prototype.
\end{ReviewerComment}
%
\begin{Answer}
The manner of the PID control and the gain tuning has been described more accurately:

``All of the utilized heuristics are combined and applied simultaneously, 
i.e.\ superimposed on the gait trajectories in the abstract space. 
The closed-loop gait is significantly more stable than the open-loop gait, 
and allows for fast walking of the robot. The strengths of the gait lies in its
simplicity. As the single feedback signal comes from the attitude 
estimation measured with the on-board IMU, the gait will work on low-cost platforms
with imprecise actuation or lacking the necessary sensors to estimate ground reaction forces, 
such as the NimbRo-OP2X. The limitation of the gait also stems from this, as every corrective action
requires gains tuned on a per-robot basis for them to contribute to the overall balance.
As manual tuning requires specialist knowledge on the behaviour of the corrective actions~(as per Allgeuer and Behnke: ``Omnidirectional Bipedal Walking with Direct Fused Angle Feedback Mechanisms''),
the next subsection deals with a more automated approach to tuning the gains. ''

A more precise description regarding the speed-up and slow-down gains has been provided, in combination with how the desired gait frequency is modified by these gains.

``The slow-down gain is selected to avoid premature stepping during a disturbance, 
effectively lowering the gait frequency, until halting it when the robot is tipping outwards.
Opposite to that, the speed-up gain increases the gait frequency when the robot
is tipping inwards to place the swing foot in time for it to make proper contact with the ground.''
\end{Answer}
%
%


%
%
\begin{ReviewerComment}{3}
In section 4.4, it is unclear whether the authors actually utilised floating-base robot models in their simulations, or whether this was eschewed to mitigate complexity. Introducing body-geometry approximations does not immediately imply the exclusion of floating-base models. This point needs further elucidation.
\end{ReviewerComment}
%
\begin{Answer}
Statements on section 4.4 have been changed.
The simulations are based on floating-base models. 
The geometry approximation is only used for reducing the complexity of the contacts.
\end{Answer}
%
%
%
\begin{ReviewerComment}{3}
	Given that there will always be a disparity between the simulated parameters, and those of the physical world, it might be deemed counterintuitive to tune the simulation gains until a close resemblance between real and simulated tracking error levels can be achieved. It would perhaps be preferable to contrast the real control signal, with that predicted in simulation, so as to ascertain that similar tracking errors can only be acquired when using comparable control input magnitudes.
\end{ReviewerComment}
%
\begin{Answer}
	More discussion about this section of the paper was added.
	
	Hwangbo et al.~[49] have demonstrated that learning the actuator model (input to output mapping) plays a key role for sim-to-real transfer.
	Similarly,
	we tune the gains of the controllers to obtain similar tracking errors as the real robot actuators~[12],
	such that the actuator model with the controller together produce a similar control output as the real actuators given the same control input.
	In this manner, the difference between the simulation model and the real actuators is reduced and the complex actuator modeling is avoided.
\end{Answer}
%
%

%
%
\begin{ReviewerComment}{3}
	Sub-section 5.2 is concerned with the system's stability, although the notion of stability is quite broad and there is a sciential chasm between the different uses of this term. When scrutinising the contents of this section, one merely observes the presence of phase plots, as opposed to CoP/ZMP measurements, Poincaré return maps, or Lyapunov functions. Therefore, the authors should pinpoint the exact type of stability that they are referring to.
\end{ReviewerComment}
%
\begin{Answer}
	We have provided an explanation on how the stability is measured:

``For the following experiments, we evaluate the locomotion stability with respect to the fused angle deviations. Due to the low-cost nature of the NimbRo-OP2X, the available feedback during locomotion is joint position sensing and attitude estimation. Without measuring ground reaction forces, utilizing indicators such as ZMP, is not possible. Although using CoM and ZMP estimates through inverse-dynamics based on joint position feedback is theoretically possible, it has been largely inaccurate in our experience. Therefore the verification of stability is based solely on the IMU measurements. A maximum angle for the fused pitch and fused roll of the trunk are established, where exceeding these values results in the robot tipping over and falling, despite any corrective actions taken. The measurements taken are then represented in the form of phase plots, which accurately represent the system behavior.''
\end{Answer}
%
%


%
%
\begin{ReviewerComment}{3}
	Some linguistic inconsistencies should be removed for clarity. Segments of the phrases, sentences, or lines that could be amended to improve clarity, are provided below: [...]
\end{ReviewerComment}
%
\begin{Answer}
	All of the linguistic inconsistencies and unclarities from the list have been amended, which we believe results in a more refined and understandable text.
\end{Answer}
%
%



%



